Can Large Vision-Language Models Correct Semantic Grounding Errors By Themselves?

Enhancing semantic grounding abilities in Vision-Language Models (VLMs) often involves collecting domain-specific training data, refining the network architectures, or modifying the training recipes. In this work, we venture into an orthogonal direction and explore whether VLMs can improve their semantic grounding by "receiving" feedback, without requiring in-domain data, fine-tuning, or modifications to the network architectures. We systematically analyze this hypothesis using a feedback mechanism composed of a binary signal. We find that if prompted appropriately, VLMs can utilize feedback both in a single step and iteratively, showcasing the potential of feedback as an alternative technique to improve grounding in internet-scale VLMs. Furthermore, VLMs, like LLMs, struggle to self-correct errors out-of-the-box. However, we find that this issue can be mitigated via a binary verification mechanism. Finally, we explore the potential and limitations of amalgamating these findings and applying them iteratively to automatically enhance VLMs' grounding performance, showing grounding accuracy consistently improves using automated feedback across all models in all settings investigated. Overall, our iterative framework improves semantic grounding in VLMs by more than 15 accuracy points under noise-free feedback and up to 5 accuracy points under a simple automated binary verification mechanism. The project website is hosted at https://andrewliao11.github.io/vlms_feedback

==> eccv2024/results/full_vlms_listen_to_feedback.tex <==

\setlength{\tabcolsep}{4pt}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lrrrrr@{}}
\toprule
\multicolumn{1}{l}{}        & \multicolumn{1}{c}{LLaVA-1.6} & \multicolumn{1}{c}{LLaVA-1.5 13b} & \multicolumn{1}{c}{Vip-LLaVA 13b} & \multicolumn{1}{c}{MiniGPTv2} & \multicolumn{1}{c}{ShareGPT} \\ \midrule
\textit{Base predictions}   &                               & 35.86                             & 35.86                             &                               &                               \\
+ Binary feedback           &                               &                                   &                                   &                               &                               \\
+ Class label feedback      &                               & 94.80                             &                                   &                               &                               \\ \bottomrule
\end{tabular}%
}\vspace{1mm}
\caption{\textbf{$\text{Acc.}$ with different feedback types.}}
\label{tab:feedback_type}
\end{table}



==> eccv2024/results/vlms_as_listener.tex <==

\setlength{\tabcolsep}{4pt}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lrrrrr@{}}
\toprule
\multicolumn{1}{l}{}        & \multicolumn{1}{c}{LLaVA-1.6} & \multicolumn{1}{c}{LLaVA-1.5 13b} & \multicolumn{1}{c}{Vip-LLaVA 13b} & \multicolumn{1}{c}{MiniGPTv2} & \multicolumn{1}{c}{ShareGPT} \\ \midrule
\textit{Base predictions}   &                               & 35.86                             & 35.86                             &                               &                               \\
+ Binary feedback           &                               &                                   &                                   &                               &                               \\
+ Class label feedback      &                               & 94.80                             &                                   &                               &                               \\ \bottomrule
\end{tabular}%
}\vspace{1mm}
\caption{\textbf{$\text{Acc.}$ with different feedback types.}}
\label{tab:feedback_type}
\end{table}



==> eccv2024/results/vlms_as_listener/feedback_types.tex <==



\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lrrr@{}}
\toprule
\multicolumn{1}{l}{}         & \multicolumn{1}{c}{LLaVA-1.5} & \multicolumn{1}{c}{Vip-LLaVA}  & \multicolumn{1}{c}{CogAgent} \\ \midrule
\rowcolor[HTML]{EFEFEF} \textit{Base predictions}   & 35.86                             & 35.86                             &                               15.98\\
+ Binary feedback           & 41.04&                                   40.36&                               16.25\\
+ Class label feedback      & 94.80                             & 74.99&                               77.04\\ \bottomrule
\end{tabular}%
}\vspace{1mm}
\caption{\textbf{$Acc_\text{grounding}$ with noise-free binary or class label types of feedback.} $\dagger$: results averaged over less than 3 seeds.}
\label{tab:feedback_type}
\end{table}



==> eccv2024/results/vlms_as_listener/textual_and_visual_prompt.tex <==
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lrrrrr@{}}
\toprule
   \multicolumn{1}{c}{}                                 & \multicolumn{1}{c}{Zero-shot CoT} & \multicolumn{1}{c}{Visual prompt}  & \multicolumn{1}{c}{LLaVA-1.5} & \multicolumn{1}{c}{Vip-LLaVA}  & \multicolumn{1}{c}{CogAgent} \\ \midrule
\rowcolor[HTML]{EFEFEF} 
\textit{Base predictions}           & No                                    & No                                & 35.86                             & 35.86                             &                              15.98\\
 & No& No& 41.04& 40.36&16.25\\
                                    & Yes& No&                                   43.3&                                   42&                              18.23\\
                                    & Yes                                   & SoM                               &                                   42.41&                                   44.53&                              18.64\\
\multirow{-4}{*}{+ Binary feedback}& Yes                                   & Red circle                        &                                   \textbf{45.38}&                                   \textbf{45.21}&                              \textbf{19.46}\\ \bottomrule
\end{tabular}%
}\vspace{1mm}
\caption{\textbf{Feedback with textual and visual prompts improve grounding Acc. }}
\label{tab:textual_and_visual_prompt}
\end{table}

==> eccv2024/results/vlms_binary.tex <==
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}llrrrrrrr@{}}
\toprule
VLM                        & Visual prompt & 0-shot CoT & Self-consistency & Feedback Acc. @ R0 & Acc. @ R0         & Acc. @ R1 & Acc. @ R2 & Acc. @ R3 \\ \midrule
\multirow{6}{*}{LLaVA-1.5} & crop          & X          & X                & 68                 & 35.45             & 38.52     & 38.93     & 38.93     \\
                           & red circle    & X          & X                & 57.2               & 35.45             & 39.13     & 39.54     & 40.16     \\
                           & crop          & V          & X                & 62.1               & 35.45             & 36.47     & 36.88     & 36.27     \\
                           & red circle    & V          & X                & 55.5               & 35.45             & 38.52     & 37.29     & 37.5      \\
                           & crop          & V          & V                & 68.4               & 35.45             & 37.09     & 36.88     & 38.11     \\
                           & red circle    & V          & V                &                    &                   &           &           &           \\ \midrule
\multirow{4}{*}{Vip-LLaVA} & crop          & X          & X                & 64.1               & 35.45$^{\dagger}$ & 34.42     & 36.68     & 37.09     \\
                           & red circle    & X          & X                &                    & 35.45$^{\dagger}$ &           &           &           \\
                           & crop          & V          & X                & 73.2               & 35.45$^{\dagger}$ & 39.54     & 41.18     & 40.57     \\
                           & red circle    & V          & X                &                    & 35.45$^{\dagger}$ &           &           &           \\ \bottomrule
\end{tabular}%
}\vspace{1mm}
\caption{\textbf{VLM correction setting}: 1) maximum boxes per VLM forward is 5 2) conditional generation to encourage instruction following. 
\textbf{Column name explained}: 0-shot CoT~\cite{zero_shot_cot}: we add ``Let's look closer to the image and think step by step'' at the beginning of the VLM responses. Self-consistency~\cite{self_consistency_cot}: draw multiple samples from VLMs and perform the majority vote. 
$^\dagger$: Vip-LLaVA improves over ``LLaVA-classified'' labels. Ideally, we should use ``Vip-LLaVA-classified'' labels.}
\label{tab:vlms_provide_binary}
\end{table}

==> eccv2024/results/vlms_self_correct.tex <==

\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
VLM                        & \#boxes per VLM forward & Feedback Acc. @ R0 & Acc. @ R0         & Acc. @ R1 & Acc. @ R2 & Acc. @ R3 \\ \midrule
\multirow{2}{*}{LLaVA-1.5} & 1                       & 56.8               & 35.45             & 32.37     & 30.53     & 27.66     \\
                           & 5                       & 47.1               & 35.45             & 36.06     & 38.11     & 38.73     \\ \midrule
\multirow{2}{*}{Vip-LLaVA} & 1                       &                    & 35.45$^{\dagger}$ &           &           &           \\
                           & 5                       &                    & 35.45$^{\dagger}$ &           &           &           \\ \bottomrule
\end{tabular}%
}\vspace{1mm}
\caption{Setting: Ask VLMs to improve itself by having another round of conversation starting with ``Carefully review and refine your answer...''
$^\dagger$: Vip-LLaVA improves over ``LLaVA-classified'' labels. Ideally, we should use ``Vip-LLaVA-classified'' labels.}
\label{tab:vlms_self_correct}
\end{table}

==> eccv2024/results/vlms_with_multitasking.tex <==
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}llllll@{}}
\toprule
VLM                        & Feedback   & Acc. @ R0 & Acc. @ R1 & Acc. @ R2 & Acc. @ R3 \\ \midrule
\multirow{3}{*}{LLaVA}     & Binary     &           &           &           &           \\
                           & Choices    &           &           &           &           \\
                           & Class name &           &           &           &           \\ \midrule
\multirow{3}{*}{MiniGPTv2} & Binary     &           &           &           &           \\
                           & Choices    &           &           &           &           \\
                           & Class name &           &           &           &           \\ \bottomrule
\end{tabular}%
}\vspace{1mm}
\caption{\textbf{VLMs's semantic grounding performances fall when multitasking.}}
\label{tab:my-table}
\end{table}

==> eccv2024/results/vlms_with_various_feedback.tex <==
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lrrrrrrr@{}}
\toprule
VLM                        & Feedback   & Conditional generation   & Acc. @ R0 & Acc. @ R1 & Acc. @ R2 & Acc. @ R3 \\ \midrule
\multirow{2}{*}{LLaVA-1.5} & Binary     & V                        & 35.45     & 45.49     & 47.33     & 48.15     \\
                           & Binary     & X                        & 35.45     &           &           &           \\ \midrule
\multirow{2}{*}{Vip-LLaVA} & Binary     & V                        & 35.45$^{\dagger}$     & 45.9      & 48.15     & 49.18     \\
                           & Binary     & X                        & 35.45$^{\dagger}$     &           &           &           \\ \bottomrule
\end{tabular}%
}\vspace{1mm}
\caption{\textbf{VLM follows feedback to improve semantic classification.} Setting: 1) maximum boxes per VLM forward is 5.
$^\dagger$: Vip-LLaVA improves over ``LLaVA-classified'' labels. Ideally, we should use ``Vip-LLaVA-classified'' labels.} 
\label{tab:vlm_follow_feedbacl_gt}
\end{table}


==> eccv2024/sections/discussion.tex <==


How to generate binary signals from off the shelf model


Model: SSL feature extractor at image-region levels, CLIP


Anchor from the training set. For each class, you have multiple prototypes.

During inference,  we have the bounding box
For each object of interest, we extract features and compute similarity prototype


noise-free experiment
 visual prompting analysis.
 analyse multiple VLMs.
 we have the baseline standard prompting, and we reach to conlusion that with this it doesnt improve so much.
 we come up with this  new way after the analyzis of doing the conditional promptiong

automatic-feedback: we want to verify if this applies to noisy environment where the verifier is not human feedback.

if this is great and it works, then great!
if this does not work, we introduce gt signal + noise.


verifier using clip:
classes,bbxoes= VLM_prediction
region_crops=extract_region_crops(bboxes) # where region_crops = # of bboxes.
for text,region_crop in zip(classes,region_crops):
    similarity_score.append(CLIP(text, region crop))

similarity_score>0.8 no issue
lower feedback

verifier using Llava on crops:
classes,bbxoes= VLM_prediction
region_crops=extract_region_crops(bboxes) # where region_crops = # of bboxes.
for text,region_crop in zip(classes,region_crops):
    yes_no_answer=LLava("Answer YES or NO. Does this image contain a "+text, region crop))
    answers.append(yes_no_answer)
    





Time:
Wed 21
Binary choice option.
Friday 23, we know if the auto-verifier works.

Wed 28
Wed 6 (deadline)

Q:why doing this if LLava already uses CLIP
A: you are using clip at region level now for the verification. 

    



==> eccv2024/sections/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\bm{\epsilon}}}
\def\rvtheta{{\bm{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\vpi{{\bm{\pi}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\px}{p(\mathbf{x})}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

%denoiser
\newcommand{\dmparam}{\vtheta}
\newcommand{\denoiser}{\rvepsilon_{\dmparam}}
%generator.
\newcommand{\gparam}{\bm{\phi}}
% \newcommand{\gparam}{\bm{\Theta}}
\newcommand{\gnet}{g_{\gparam}}
%
\newcommand{\encoder}{\gE}
\newcommand{\decoder}{\gD}
%
\newcommand{\encodertext}{\gE_{\textnormal{text}}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\newcommand{\img}{{\mathbf{I}}}
\newcommand{\imgRendered}{{\hat {\mathbf{I}}}}
\newcommand{\imgReference}{{\mathbf{I}_r}}
\newcommand{\imgReferenceCropped}{{\mathbf{I}_r^c}}
\newcommand{\imgPatch}{{\mathbf{I}_p}}
\newcommand{\imgPatchRendered}{\hat{\mathbf{I}}^p}

\newcommand{\globalText}{{\textit{"A photo of sks"}}}
\newcommand{\localText}{{\textit{"A photo of sks, cropped"}}}

% \renewcommand{\subsubsectionautorefname}{\S}
% \renewcommand{\subsectionautorefname}{\S}
% \renewcommand{\sectionautorefname}{\S}

